TexPose: Neural Texture Learning for Self-Supervised 6D Object Pose Estimation

In this paper, we introduce neural texture learning for 6D object pose estimation from synthetic data and a few unlabelled real images. Our major contribution is a novel learning scheme which removes the drawbacks of previous works, namely the strong dependency on co-modalities or additional refinement. These have been previously necessary to provide training signals for convergence. We formulate such a scheme as two sub-optimisation problems on texture learning and pose learning. We separately learn to predict realistic texture of objects from real image collections and learn pose estimation from pixel-perfect synthetic data. Combining these two capabilities allows then to synthesise photorealistic novel views to supervise the pose estimator with accurate geometry. To alleviate pose noise and segmentation imperfection present during the texture learning phase, we propose a surfel-based adversarial training loss together with texture regularisation from synthetic data. We demonstrate that the proposed approach significantly outperforms the recent state-of-the-art methods without ground-truth pose annotations and demonstrates substantial generalisation improvements towards unseen scenes. Remarkably, our scheme improves the adopted pose estimators substantially even when initialised with much inferior performance.

==> tables/ablation_eqn1_eqn2.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}[h]
\begin{center}
\caption{Ablation study of the individual effect of each component from Eqn.1 and Eqn.2 on partial objects. *: objects with symmetry.}
\label{table:ablative_eqn12}

\scriptsize
\scalebox{1.4}{

\begin{tabular}{|c | c | c c c c c c | c|}
\hline
\text{Variant} & \text{Objective} & Ape & Cat & Duck & Glue* & Holep. & Phone & Average \\
\hline
 M1 & w/o self-sup  & 50.9 & 79.9 & 24.6 &  81.2 & 41.9 & 64.3 & 57.1   \\
 M2 & Opt. Pose  &  \textbf{85.8} & 91.5 & 61.9 &  93.3 & 32.1 & \textbf{94.8} & 76.5   \\

\hline
M3 & Eqn. 1 (Self6D++) &	76.0	& 85.6	& 56.5	& 92.2 &	35.4 &	91.8 &	72.9 \\
M4 & Eqn. 1 + Eqn. 2.2 & 64.5 &	91.1 &	52.1 &	96.8 &	43.7 &	84.7 &	72.1 \\
M5 & Eqn. 2 + Eqn. 1.1  & 81.7 & 95.5 & 79.6 &  94.5 & 75.9 & 87.3 & \textbf{85.7}   \\
M6 & Eqn. 1 + Eqn. 2 & 81.5 & \textbf{95.8} & 78.2 &  \textbf{98.1} & 67.9 & 90.7 & 85.3   \\
M7 & Eqn. 2 (Ours) &   80.9 & 92.6 & \textbf{83.4}  & 93.4 &  \textbf{79.3} & 78.9 & 84.7   \\

\hline
\end{tabular}}
\end{center}
\end{table}

==> tables/ablation_iters.tex <==
\setlength{\tabcolsep}{3.5pt}

\begin{table}[h]
\begin{center}
\caption{Ablation study  of number of iterations on partial objects. *: objects with symmetry.}
\label{table:ablative_iters}
\scriptsize
\scalebox{1.4}{

\begin{tabular}{| c | c c c c c c | c|}
\hline
\text{\# Iterations} & Ape & Cat & Duck & Glue* & Holep. & Phone & Average \\
\hline
w/o self-sup  & 50.9 & 79.9 & 24.6 &  81.2 & 41.9 & 64.3 & 57.1   \\
1             & \textbf{80.9} & 92.6 & 83.4  & 93.4 & \textbf{79.3} & 78.9 & 84.7   \\
2             & 77.9 & \textbf{93.7} & \textbf{83.6}  &  \textbf{95.0}    & 76.0 & \textbf{83.3} & \textbf{84.9}\\
% 3             & -  & - & - & - & - & - & -   \\
\hline
\end{tabular}}
\end{center}
% \vspace*{-3mm}%01.03
\end{table}

\vspace*{-1mm}

==> tables/cad_model.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}[h]
\begin{center}
\scriptsize
\caption{Ablation study of the necessity of "split" scheme on partial objects. *: objects with symmetry.}
\label{table:split}
\scalebox{1.4}{

\begin{tabular}{| c | c c c c c c | c|}
\hline
\text{Training strategy} & Ape & Cat & Duck & Glue* & Holep. & Phone & Average \\
\hline
w/o self-sup  & 50.9 & 79.9 & 24.6 &  81.2 & 41.9 & 64.3 & 57.1   \\
w/o geo-tex split  & 25.1 & 73.1 & 45.7 &  71.4 & 27.8 & 69.4 & 52.1   \\
w/ geo-tex split (Ours)  & \textbf{80.9} & \textbf{92.6} & \textbf{83.4}  & \textbf{93.4} & \textbf{79.3} & \textbf{78.9} & \textbf{84.7}   \\
\hline
\end{tabular}}
\end{center}
\end{table}

==> tables/hb.tex <==
% \setlength{\tabcolsep}{2.7pt}
\begin{table}[!b]
\begin{center}
\caption{Evaluation results on HomebrewedDB dataset. **: used as our pretrained pose estimator before self-supervision, consistent with Self6D++. $\dagger$: Pre-process testing images with the same intrinsics as LineMOD, different from \cite{Wang_2021_self6dpp} as they directly feed raw images without scaling $\ddagger$: Self6D++ variant with depth supervision.}
\label{table:hb}
\scriptsize
\begin{tabular}{|c | c | c c c c  | c c c c |}
 
\hline
% Supervision & \multicolumn{1}{c|} {\textbf{NOL}} & \multicolumn{4}{c|}{synthetic images}&{real+syn} &\multicolumn{1}{c|}{\textbf{NOL}} &\multicolumn{2}{c|}{syn}&\multicolumn{1}{c|}{real}&\multicolumn{1}{c}{r+s} \\
Supervision & Syn & \multicolumn{4}{c|}{Syn + Self (using LineMOD)} & \multicolumn{4}{c|}{Syn + Self (using HomebrewedDB)} \\
\hline  
Method    
& GDR** $\dagger$ \cite{DBLP:conf/cvpr/0001MTJ21}   
& Sock~\etal  \cite{DBLP:conf/3dim/SockGAK20}
& DSC  \cite{DBLP:conf/cvpr/YangY021}
& Self6D++ $\dagger$ \cite{Wang_2021_self6dpp}
& \textbf{Ours} $\dagger$ 
& DSC \cite{DBLP:conf/cvpr/YangY021}
& Self6D++ \cite{Wang_2021_self6dpp}
& Self6D++ $\ddagger$ \cite{Wang_2021_self6dpp}
& \textbf{Ours} \\

\hline
Benchvise & 88.8   & 57.3 & 72.9 & 75.7  & \textbf{93.1} & 78.2  & 56.1 & 67.1 & \textbf{92.9}\\
Driller   & 92.8   & 46.6 & 40.6 & 89.4  & \textbf{94.8} & 76.2  & 97.7 & \textbf{98.0} & 94.2\\
Phone     & 78.7   & 41.5 & 18.5 & 76.8  & \textbf{79.3} & 42.9  & 85.1 & \textbf{88.2} & 81.2\\
\hline
Average   & 86.8   & 52.0 & 44.0 & 80.6  & \textbf{89.1} & 65.8  & 79.6 & 84.4 & \textbf{89.4}\\
\hline

\end{tabular}
\end{center}
\vspace*{-5mm}%01.03
\end{table}

% \setlength{\tabcolsep}{4.5pt}
% \begin{table}[t]
% \begin{center}
% \caption{Evaluation results on LineMOD. The ADD score is used except for {\it Eggbox} and {\it Glue} that use the ADI score}
% \label{table:hb}
% \scriptsize
% \begin{tabular}{|c | c | c | c c c c  | c c c c |}
 
%  \hline

% % Supervision & \multicolumn{1}{c|} {\textbf{NOL}} & \multicolumn{4}{c|}{synthetic images}&{real+syn} &\multicolumn{1}{c|}{\textbf{NOL}} &\multicolumn{2}{c|}{syn}&\multicolumn{1}{c|}{real}&\multicolumn{1}{c}{r+s} \\
% Supervision & Syn & Syn + Real & \multicolumn{4}{c|}{Syn + Self (using LineMOD)} & \multicolumn{4}{c|}{Syn + Self (using HomebrewedDB)} \\
% \hline  
% Method    & GDR  & GDR  & Sock & DSC  & Self6D++ & Ours & DSC & Self6D++ & Self6D++ (D) & Ours \\

% \hline
% Benchvise & 88.8 & 98.6 & 57.3 & 72.9 & 75.7  & 93.1 & 78.2  & 56.1 & 67.1 & 92.9\\
% Driller   & 92.8 & 97.7 & 46.6 & 40.6 & 89.4  & 94.8 & 76.2  & 97.7 & 98.0 & 94.2\\
% Phone     & 78.7 & 85.1 & 41.5 & 18.5 & 76.8  & 79.3 & 42.9  & 85.1 & 88.2 & 81.2\\
% \hline
% Average   & 86.8 & 93.8 & 52.0 & 44.0 & 80.6  & 89.1 & 65.8  & 79.6 & 84.4 & 89.4\\
% \hline

% \end{tabular}
% \end{center}
% %01.03\vspace*{-3mm}%01.03
% \end{table}



==> tables/hyperparams.tex <==
\setlength{\tabcolsep}{8pt}
\begin{table}[htb]
\begin{center}
\caption{All chosen hyperparameters for the experiments.}
\label{table:hparams}
\scriptsize
\scalebox{1.5}{
\begin{tabular}{| c | c c c c c c|}
\hline
Factor & $\lambda_m$ & $\lambda_d$&  $\lambda_t$ & $\lambda_{fg}$ & $\lambda_{adv}$ & $\lambda_{reg}$ \\
\hline

Value & 0.1 & 0.1 & 0.01 & 5 & 0.1 & 0.01  \\

\hline
\end{tabular}}
\end{center}
%01.03\vspace*{-3mm}%01.03
\end{table}

==> tables/lm_dpodv2_partial.tex <==
\setlength{\tabcolsep}{3.5pt}

\begin{table}[h]
\begin{center}
\caption{Evaluation results on partial objects from LineMOD dataset tested with our re-implementation of DPODv2~\cite{shugurov2021dpodv2} pose estimator. Results of DPODv2-LB and DPODv2-UB are slightly different from the original paper.}
\label{table:lm_dpodv2}
\scriptsize
\scalebox{1.3}{

\begin{tabular}{| c | c c c c c c | c|}
\hline
\text{Methods} & Ape & B.vise & Cat & Duck & Holep. & Phone & Average \\
\hline
DPODv2-LB        &  59.7 & 85.0 & 79.3 & 51.2 & 28.1 & 69.7 &	62.1 \\
DPODv2-Self Sup. &  \textbf{77.8} & \textbf{98.4} & \textbf{90.6}  & \textbf{72.9} & \textbf{64.4} & \textbf{85.6} & \textbf{81.6}   \\
\hline
DPODv2-UB     &  80.1 & 97.6 & 95.1 & 80.5  & 75.5 & 96.5  & 87.5  \\
% 3             & -  & - & - & - & - & - & -   \\
\hline
\end{tabular}}
\end{center}
% \vspace*{-3mm}%01.03
\end{table}

\vspace*{-1mm}

==> tables/lm_random_seed.tex <==
\setlength{\tabcolsep}{2.0pt}

\begin{table}[htb]
\begin{center}
\caption{Evaluation results on LineMOD dataset with random seeds.}
\label{table:lm_seed}
\scalebox{0.9}{
\begin{tabular}{| c | c c c c c c c c c c c c c| c|}
\hline
\text{Seed} & Ape & B.vise & Camera & Can & Cat & Driller & Duck & Eggbox & Glue & Holep. & Iron & Lamp & Phone & Average \\
\hline
\# 1       &  81.6 & 98.2 & 96.2 & 99.9 & 90.9 & 98.6 &	83.0 &  92.5 & 96.4 & 78.2 & 99.6 & 97.7 & 73.2 & 91.2 \\
\# 2       &  80.9 & 99.0 & 94.8 & 99.7 & 92.6 & 97.4 & 83.4 &  94.9 & 93.4 & 79.3 & 99.8 & 98.3 & 78.9 & 91.7 \\
\# 3       &  79.3 & 98.5 & 95.5 & 99.7 & 92.8 & 96.7 &	84.2 &  93.2 & 94.5 & 77.6 & 99.9 & 98.2 & 77.9 & 91.4 \\
% 3             & -  & - & - & - & - & - & -   \\
\hline
\end{tabular}}
\end{center}
% \vspace*{-3mm}%01.03
\end{table}

\vspace*{-1mm}




==> tables/lmo.tex <==
% \setlength{\tabcolsep}{3.5pt}
% \begin{table}[t]
% \begin{center}
% \caption{Evaluation results on LineMOD. The ADD score is used except for {\it Eggbox} and {\it Glue} that use the ADI score}
% \label{table:lmo}
% \scriptsize
% \begin{tabular}{c | c c c c c | c c c  c c | c c  c c c c}

% % \hline
% % Supervision & \multicolumn{16}{c}{Supervision modality used in real domain}\\
% % \hline
% %  Depth & -  & - & - & - & - & -   & -  & - & - & - & - & - & - & - & - & -\\
 
% %  Pose Refiner & -  & - & - & - & - & -   & -  & - & - & - & - & - & - & - & - & -\\
 
% %  Weak labels & -  & - & - & - & - & -   & -  & - & - & - & - & - & - & - & - & -\\
 
% %  GT Pose labels & -  & - & - & - & - & -   & -  & - & - & - & - & - & - & - & - & -\\
  
% %  GT Pose labels & -  & \checkmark & \checkmark & \checkmark & \checkmark &\checkmark   & -  & \checkmark & \checkmark & - & \checkmark & - & \checkmark & - & \checkmark & -\\
 
%  \hline

% % Supervision & \multicolumn{1}{c|} {\textbf{NOL}} & \multicolumn{4}{c|}{synthetic images}&{real+syn} &\multicolumn{1}{c|}{\textbf{NOL}} &\multicolumn{2}{c|}{syn}&\multicolumn{1}{c|}{real}&\multicolumn{1}{c}{r+s} \\
% Supervision & \multicolumn{5}{c|}{Syn} & \multicolumn{5}{c|}{Syn + Real} & \multicolumn{6}{c}{Syn + Self} \\
% \hline  


% Method & A & B  & C &  D & E & F & G & H & I & J & K & I & J & K & I & J\\
% \hline
% Ape  & - & - & - & - & - &  - & - &- &- & -& - &- &- & - &- &-\\
% Can  & - & - & - & - & - &  - & - &- &- & -& - &- &- & - &- &-\\
% Cat  & - & - & - & - & - &  - & - &- &- & -& - &- &- & - &- &-\\
% Driller  & - & - & - & - & - &  - & - &- &- & -& - &- &- & - &- &-\\
% Duck  & - & - & - & - & - &  - & - &- &- & -& - &- &- & - &- &-\\
% Eggbox  & - & - & - & - & - &  - & - &- &- & -& - &- &- & - &- &-\\
% Glue  & - & - & - & - & - &  - & - &- &- & -& - &- &- & - &- &-\\
% Holep. & - & - & - & - & - &  - & - &- &- & -& - &- &- & - &- &-\\
% \hline
% Average  & - & - & - & - & - &  - & - &- &- & -& - &- &- & - &- &-\\ 
% \hline

% \end{tabular}
% \end{center}
% %01.03\vspace*{-3mm}%01.03
% \end{table}

\setlength{\tabcolsep}{3 pt}
\begin{table}[h]
\begin{center}
\caption{Evaluation results on Occluded LineMOD dataset. *: objects with symmetry. **: used as our pretrained pose estimator before self-supervision, consistent with Self6D++. $\dagger$:re-implemented version from \cite{Wang_2021_self6dpp}, used as supervision source for Self6D++. $\ddagger$: variant with depth supervision.}
\label{table:lmo}
\scriptsize
\begin{tabular}{|c | c c c c| c | c c c c c c|}
 
 \hline

Supervision & \multicolumn{4}{c|}{Syn} & Syn + Real &\multicolumn{6}{c|}{Syn + Self} \\
\hline  


\multirow{2}{*}{Methods}  & 
CDPNv2  & 
CosyPose   & 
GDR-LB**   & 
DeepIM $\dagger$  & 
GDR-UB   & 
Self6D  & 
Sock~\etal  & 
DSC   & 
Self6D++   & 
Self6D++$\ddagger$   & 
\multirow{2}{*}{\textbf{Ours}} \\

  & 
\cite{DBLP:conf/iccv/LiWJ19} & 
\cite{DBLP:conf/eccv/LabbeCAS20}  & 
\cite{DBLP:conf/cvpr/0001MTJ21} & 
\cite{DBLP:journals/ijcv/LiWJXF20}& 
\cite{DBLP:conf/cvpr/0001MTJ21} & 
\cite{DBLP:conf/eccv/WangMSJNT20}& 
\cite{DBLP:conf/3dim/SockGAK20} & 
\cite{DBLP:conf/cvpr/YangY021} & 
\cite{Wang_2021_self6dpp} & 
\cite{Wang_2021_self6dpp} & 
\\
\hline
Ape       & 20.6 & 44.0 & 44.0 & \textbf{53.7} & 53.7  & 13.7 & 12.0 & 9.1 & 57.7 & 59.4 & \textbf{60.5} \\
Can       & 64.8 & 69.9 & 83.9 & \textbf{97.0} & 93.5 & 43.2 & 27.5 & 21.1 & 95.0 & \textbf{96.5} & 93.4 \\
Cat       & 24.0 & 42.1 & 49.1 & \textbf{60.2} & 57.3 & 18.7 & 12.0 & 26.0 & 52.6 & \textbf{60.8} & 56.1 \\
Driller   & 60.0 & 67.5 & 88.5 & \textbf{96.5} & 91.5 & 32.5 & 20.5 & 33.5 & 90.5 & 92.0 & \textbf{92.5} \\
Duck      & 42.2 & \textbf{47.8} & 15.0 & 27.8 & 71.7 & 14.4 & 23.0 & 12.2 & 26.7 & 30.6 & \textbf{55.5} \\
Eggbox*    & 40.0 & 24.4 & 33.9 & \textbf{51.1}& 57.8  & 57.8 & 25.1 & 39.4 & 45.0 & \textbf{51.1} & 46.0 \\
Glue*      & 66.4 & 60.0 & 75.0 & \textbf{89.3}& 88.6  & 54.3 & 27.0 & 37.0 & 87.1 & \textbf{88.6} & 82.8 \\
Holep.    & \textbf{42.0} & 17.5 & 34.0 & 24.5 & 81.0 & 22.0 & 35.0 & 20.4 & 23.5 & 38.5 & \textbf{46.5} \\
\hline
Average   & 45.0 & 46.7 & 52.9 & \textbf{62.5} &  74.4 & 32.1 & 22.8 & 24.8 & 59.8 & 64.7 & \textbf{66.7} \\ 
\hline

\end{tabular}
\end{center}
%01.03\vspace*{-3mm}%01.03
\end{table}

==> tables/ycb.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}[h]
\begin{center}
\scriptsize
\caption{Evaluation results on Occluded YCB-Video dataset.}
\label{table:ycb}

\begin{tabular}{| c | c c |c c || c c |}
\hline
   & \multicolumn{2}{c|}{Syn} & \multicolumn{2}{c||}{Syn + Self} & \multicolumn{2}{c|}{Syn + Real} \\
  \hline
    Metric    & AUC/ADD-S & AUC/ADD(-S) & AUC/ADD-S & AUC/ADD(-S) & AUC/ADD-S & AUC/ADD(-S) \\
  \hline

  006\_mustard\_bottle & \textbf{97.5} & 91.9 & 96.3 &  \textbf{99.5} & 100.0 &  94.7  \\
  007\_tuna\_fish\_can & 96.0 & 86.7 & \textbf{97.3} &  \textbf{89.3} & 99.9 &  97   \\
  021\_bleach\_cleanser & \textbf{90.5} & 80.0 & 89.5 &  \textbf{80.3} & 91.2 &  81.9 \\
  035\_power\_drill& 94.7 & 84.6 & \textbf{96.0} &  \textbf{88.3} & 99.7 & 93.6   \\
  040\_large\_marker  & 82.9 & 70.5 & \textbf{88.2} &  \textbf{77.3} & 93 &  81.7  \\
  \hline
  Average & 92.3 & 82.7 & \textbf{93.4} &  \textbf{86.9} & 96.7 &  89.7  \\
  
\hline
\end{tabular}
\end{center}
\end{table}
